On the Optimality of Rate Balancing for Max-Min Fair Multicasting

The max-min fair (MMF) multicasting problem is known to be NP-hard. In this work, we analytically derive the optimal solution to this NP-hard problem and establish the equivalence between rate balancing and the optimal MMF multicasting solution under certain conditions. Based on this theoretical insight, we propose a low-complexity algorithm for MMF multicasting that yields closed-form solutions. Simulation results validate our analysis and demonstrate that the proposed algorithm outperforms the state-of-the-art methods while being computationally more efficient.

==> hist_M8K10.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=15.5in,
height=8.108in,
 width= 1.0\linewidth,   % full text width
height=0.6\linewidth, 
at={(2.6in,1.094in)},
scale only axis,
bar shift auto,
xmin=0.507692307692308,
xmax=10.4923076923077,
xtick={ 1,  2,  3,  4,  5,  6,  7,  8,  9, 10},
xlabel style={font=\color{white!15!black}},
xlabel={User Index},
ymin=0,
ymax=20,
ylabel style={font=\color{white!15!black}},
ylabel={Value},
axis background/.style={fill=white},
%title style={font=\bfseries},
%title={M = 8; K = 10; Pt = 10 dB},
xmajorgrids,
ymajorgrids,
legend style={at={(0,0.9)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black, row sep=-0.05cm},
legend columns=3
]
\addplot[ybar, bar width=0.123, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
1	5.55621583356001\\
2	5.55621583494007\\
3	5.55621584533406\\
4	5.55621583535791\\
5	7.06777424953624\\
6	5.55621583400076\\
7	5.55621583513794\\
8	5.55621583366894\\
9	5.55621583993448\\
10	9.1604462930724\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.507692307692308	0\\
10.4923076923077	0\\
};
\addlegendentry{CVX Relaxed}

\addplot[ybar, bar width=0.1023, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
1	3.3680585130821\\
2	4.19415858603775\\
3	5.60301166612324\\
4	3.38926975135216\\
5	6.07828491474623\\
6	14.1066652026114\\
7	4.55920808064341\\
8	3.34925313841318\\
9	5.05531687174946\\
10	24.0465051137674\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.507692307692308	0\\
10.4923076923077	0\\
};
\addlegendentry{CVX Rand}

\addplot[ybar, bar width=0.123, fill=mycolor3, draw=black, area legend] table[row sep=crcr] {%
1	4.06940018289819\\
2	4.06873930875235\\
3	4.07092484775513\\
4	4.07011970052058\\
5	4.06870443483478\\
6	4.06998903351764\\
7	4.06863126733744\\
8	4.06864921134244\\
9	4.06933424160566\\
10	4.07123212043806\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.507692307692308	0\\
10.4923076923077	0\\
};
\addlegendentry{Algo Rate}

\addplot[ybar, bar width=0.123, fill=mycolor4, draw=black, area legend] table[row sep=crcr] {%
1	3.63576494437721\\
2	5.85001446311461\\
3	11.4794248651111\\
4	4.95495867879186\\
5	13.6301590338444\\
6	4.22377169006663\\
7	3.55695035323502\\
8	3.65912597334448\\
9	9.02480377017555\\
10	5.24811647386253\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.507692307692308	0\\
10.4923076923077	0\\
};
\addlegendentry{ADMM}

\addplot[ybar, bar width=0.123, fill=mycolor5, draw=black, area legend] table[row sep=crcr] {%
1	5.96033864201002\\
2	2.53735064996668\\
3	3.7889182911107\\
4	13.3789123007695\\
5	2.15884413361539\\
6	1.36137623781415\\
7	2.24005369694234\\
8	4.37520145838743\\
9	1.36137597998658\\
10	3.25475105005662\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.507692307692308	0\\
10.4923076923077	0\\
};
\addlegendentry{SINR Inc}

\end{axis}
\end{tikzpicture}%
